Non-Zero Sum Games for Reactive Synthesis

In this invited contribution, we summarize new solution concepts useful for the synthesis of reactive systems that we have introduced in several recent publications. These solution concepts are developed in the context of non-zero sum games played on graphs. They are part of the contributions obtained in the inVEST project funded by the European Research Council.

==> commands.tex <==
\newcommand{\playerOne}{\ensuremath{\mathcal{P}_{1}} }\newcommand{\abs}[1]{\ensuremath{\vert #1\vert} }
\newcommand{\mn}[1]{$\bigstar$\marginpar{$\bigstar$ #1}}
\newcommand{\states}{\ensuremath{S} }
\newcommand{\state}{\ensuremath{s} }
\newcommand{\statesOne}{\ensuremath{S_{1}} }
\newcommand{\succStates}[1]{\ensuremath{{\sf Succ}(#1)} }
\newcommand{\succStatesFull}{\ensuremath{\succStates{\state} = \{ \state' \in \states \mid (\state, \state') \in \edges\}} }
\newcommand{\supp}{\ensuremath{{\sf Supp}} }
\newcommand{\initState}{\ensuremath{s_{{\sf init}}} }
\newcommand{\edges}{\ensuremath{E} }
\newcommand{\edge}{\ensuremath{e} }
%\newcommand{\weight}{\ensuremath{w} }
\newcommand{\mpTrans}{\ensuremath{\Delta} }
\newcommand{\markovProcess}{\ensuremath{{M} }}
\newcommand{\statesProb}{\ensuremath{S_{\mpTrans}} }
\newcommand{\markovProcessFull}{\ensuremath{{P = (\statesOne, \statesProb, \edges, \mpTrans, \weight)} }}
\newcommand{\dist}{\ensuremath{p} }
\newcommand{\dists}{\ensuremath{\mathcal{D}} }
\newcommand{\integ}{\ensuremath{\mathbb{Z}} }
\newcommand{\strat}{\ensuremath{\sigma} }
\newcommand*{\pr}{\mathbb{P}}
\newcommand*{\mpsup}{\ensuremath{\overline{\mathsf{MP}}}}
\newcommand*{\mpinf}{\ensuremath{\underline{\mathsf{MP}}}}
\newcommand*{\expect}{\mathbb{E}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\Inf}{\textrm{\sf Inf}}
\newcommand{\truncatedTarget}{\ensuremath{T} }
\newcommand{\truncatedSum}[1]{\ensuremath{{\sf TS}^{#1}} }
\newcommand{\discSum}[1]{\ensuremath{{\sf DS}^{#1}} }
\newcommand{\discount}{\ensuremath{\lambda} }
\newcommand{\dimension}{\ensuremath{d} }
\newcommand{\queries}{\ensuremath{q} }
\newcommand{\nat}{\ensuremath{\mathbb{N}} }
\newcommand{\rat}{\ensuremath{\mathbb{Q}} }
\newcommand{\twoCM}{\ensuremath{\mathcal{M}} }
\newcommand{\strats}{\ensuremath{\Sigma} }
\newcommand{\round}{\ensuremath{{\sf Round}_{\gamma}} }
\newcommand{\roundedDiscSum}[1]{\ensuremath{{\sf RDS}^{#1}} }
\usetikzlibrary{shapes,arrows}
